Reliable Decision from Multiple Subtasks through Threshold Optimization: Content Moderation in the Wild

Social media platforms struggle to protect users from harmful content through content moderation. These platforms have recently leveraged machine learning models to cope with the vast amount of user-generated content daily. Since moderation policies vary depending on countries and types of products, it is common to train and deploy the models per policy. However, this approach is highly inefficient, especially when the policies change, requiring dataset re-labeling and model re-training on the shifted data distribution. To alleviate this cost inefficiency, social media platforms often employ third-party content moderation services that provide prediction scores of multiple subtasks, such as predicting the existence of underage personnel, rude gestures, or weapons, instead of directly providing final moderation decisions. However, making a reliable automated moderation decision from the prediction scores of the multiple subtasks for a specific target policy has not been widely explored yet. In this study, we formulate real-world scenarios of content moderation and introduce a simple yet effective threshold optimization method that searches the optimal thresholds of the multiple subtasks to make a reliable moderation decision in a cost-effective way. Extensive experiments demonstrate that our approach shows better performance in content moderation compared to existing threshold optimization methods and heuristics.

==> algorithms/1_algorithm.tex <==
\begin{algorithm}[t]
\caption{Content Moderation as a Multiclass Classification}
\label{alg:1_content_moderation_as_a_multiclass_classification}
\begin{algorithmic}
\scriptsize
    \State {\bfseries Input:} Policy $\mathscr{p}$, Input $\mathbf{x}$.
    \State {\bfseries Output:} Appropriate class for $\mathbf{x}$ given policy $\mathscr{p}$
    \State {Define classes $R_{\mathscr{p}}$ for a multiclass classification from sub policies of $\mathscr{p}$}
    \For{$i=n_{\mathscr{p}}, \cdots, 1$}
        \If{$\mathbf{x}$ corresponds to the $(n_{\mathscr{p}} - i + 1)$-th highest priority sub policy}
            \State {\bfseries return} $r^{\mathscr{p}}_{i}$
        \EndIf
    \EndFor
    \State {\bfseries return} $r_0$
\end{algorithmic}
\end{algorithm}

==> tables/1_statistics_of_unsmile.tex <==
\begin{table}[t]
\caption{Statistics of the UnSmile dataset.}
\label{tab:1_statistics_of_unsmile}
\small
\begin{center}
\begin{tabular}{lrr}
\toprule
\multirow{2}{*}{Label} & \# of Train & \# of Validation \\
 &  Samples & Samples \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Ageism & 1,599 & 394 \\
Curse & 3,146 & 786 \\
Male & 1,347 & 334 \\
Misogyny & 1,599 & 394 \\
Other Hatred & 569 & 134 \\
Race and Nationality & 1,728 & 426 \\
Regionalism & 1,052 & 260 \\
Religion & 1,181 & 290 \\
Sexual Minority & 1,138 & 280 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
Total & 15,005 & 3,737 \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> tables/_unused_4_sota_case_2.tex <==
\begin{table}[t]
\caption{}
\label{tab:sota_case_2}
\centering
\begin{tabular}{c|l|c|c}

\toprule

Target & \multicolumn{1}{c|}{\multirow{2}{*}{Method}} & Recall \\
Precision &\\

\midrule
\multirow{9}{*}{0.9}
& Bespoke & 0.2759 \\
\cline{2-3}
& defThresh $(\tau=0.5)$ & - \\
& GreedyThresh & - \\
& SGLThresh $(\alpha=8)$ & - \\
& SGLThresh $(\alpha=32)$ & 0.2246 \\
& SGLThresh $(\alpha=128)$ & 0.2171 \\
\cline{2-3}
& TruSThresh $(\alpha=8)$ & \textbf{0.3091} \\
& TruSThresh $(\alpha=32)$ & 0.2631 \\
& TruSThresh $(\alpha=128)$ & 0.2599 \\

\midrule
\multirow{9}{*}{0.95}
& Bespoke & 0.1679 \\
\cline{2-3}
& defThresh $(\tau=0.5)$ & - \\
& GreedyThresh & - \\
& SGLThresh $(\alpha=8)$ & - \\
& SGLThresh $(\alpha=32)$ & 0.0246 \\
& SGLThresh $(\alpha=128)$ & 0.0631 \\
\cline{2-3}
& TruSThresh $(\alpha=8)$ & 0.1668 \\
& TruSThresh $(\alpha=32)$ & \textbf{0.1690} \\
& TruSThresh $(\alpha=128)$ & 0.1412 \\

\midrule
\multirow{9}{*}{0.975}
& Bespoke & 0.0235 \\
\cline{2-3}
& defThresh $(\tau=0.5)$ & - \\
& GreedyThresh & - \\
& SGLThresh $(\alpha=8)$ & - \\
& SGLThresh $(\alpha=32)$ & 0.0096 \\
& SGLThresh $(\alpha=128)$ & 0.0481 \\
\cline{2-3}
& TruSThresh $(\alpha=8)$ & \textbf{0.1444} \\
& TruSThresh $(\alpha=32)$ & 0.1348 \\
& TruSThresh $(\alpha=128)$ & 0.0995 \\

\bottomrule
\end{tabular}
\end{table}
